Multiplexed Label-Free Cytokine Sensing Using a 128x128 CMOS ISFET Array with Flexdym Microfluidic Partitioning

Cytokine-mediated inflammation disorders such as sepsis and cytokine release syndrome demand bedside multiplex panels that resolve pro- and anti-inflammatory dynamics in minutes, yet label-free FET cytokine sensors remain limited to few devices, single analytes, and PDMS packaging that sorbs small molecules and leaches oligomers. We present a CMOS platform pairing a 128 x 128 ion-sensitive field-effect transistor (ISFET) array (SkyWater 130 nm, SiN gate) with a FlexDym 4 x 1 micro-well overlay that partitions the membrane into four chemically independent regions (approximately 2,176 pixels each, square-root-of-N averaging). Two wells carry capture antibodies (anti-IL-6, anti-IL-10), one is a non-specific reference, and one tests specificity; the transduced signal is defined as the differential current relative to the reference signal (Delta I_D(W_n) - Delta I_D(W_3)). Single-analyte dose-response measurements spanning 100 fM to 10 nM successfully resolve both IL-6 and IL-10 above the non-specific detection floor, including at healthy-serum baseline concentrations. The array shows a per-pixel pH sensitivity of 1.13 microamperes per pH unit (CV approximately 14%). Across two chips, device-to-device variation is dominated by transconductance spread (g_m CV approximately 62%); a one-time per-device g_m calibration reduces analyte-measurement variance to approximately 16%. We further validate the surface functionalization, characterize device-to-device variation, and demonstrate the FlexDym integration workflow. Simultaneous multiplexed cytokine measurements resolve IL-6 (W1) and IL-10 (W2) against the chemistry-only reference (W3). At the same time, cross-specificity characterization is assessed by applying IL-6 to an anti-IL-10 well (W4), establishing a scalable label-free ISFET architecture for multiplexed cytokine sensing.

==> preamble.tex <==
\usepackage[numbers]{natbib}
\usepackage{amsmath,amssymb}
\usepackage{graphicx}
\usepackage{booktabs}
\usepackage{afterpage}
\usepackage{tabularx}
\usepackage{multirow}
\usepackage{array}
\usepackage{siunitx}
\usepackage{enumitem}
\usepackage{balance}
\usepackage{mhchem}
\usepackage{xcolor}
\usepackage{ragged2e}
\usepackage{url}
\usepackage{float}
\usepackage{subfig}
\usepackage{verbatim}   % provides the {comment} environment
\hypersetup{hidelinks}
\sisetup{detect-all,separate-uncertainty=true,range-phrase=--,range-units=single}

% --- float placement ---
\renewcommand{\topfraction}{0.9}
\renewcommand{\bottomfraction}{0.8}
\renewcommand{\textfraction}{0.07}
\renewcommand{\floatpagefraction}{0.85}
\setcounter{topnumber}{3}
\setcounter{totalnumber}{5}

% --- shorthand ---
\newcommand{\isfet}{ISFET}
\newcommand{\flexdym}{FlexDym}
\newcommand{\siN}{Si\textsubscript{3}N\textsubscript{4}}
\newcommand{\figdose}{\autoref{fig:dose_curve}(a)}
\newcommand{\figtemporal}{\autoref{fig:dose_curve}(b)}
\newcommand{\figdevvar}{\autoref{fig:dose_curve}(c)}
\newcommand{\figfluor}{\autoref{fig:chemistry}(d)}
\newcommand{\Vth}{V_{\mathrm{th}}}
\newcommand{\dVth}{\Delta V_{\mathrm{th}}}
\newcommand{\dIds}{\Delta I_{D}}
\newcommand{\lD}{\lambda_{\mathrm{D}}}
\newcommand{\etal}{\textit{et~al.}}
\newcommand{\TBD}{\textcolor{red}{\textbf{??}}}
\DeclareRobustCommand{\suppref}[1]{Supplementary Section~#1}

% ---- plateau dID at Vgs=+2 V ----
\newcommand{\platilten}{\SI{+5.40}{\micro\ampere}}
\newcommand{\platilsix}{\SI{+2.94}{\micro\ampere}}

% ---- LOD / EC50 ----
\newcommand{\LODilten}{\ensuremath{<}\,\SI{100}{fM}}
\newcommand{\LODiltenMass}{\ensuremath{<}\,\SI{1.9}{pg/mL}}
\newcommand{\LODilsix}{\SI{0.7}{pM}}
\newcommand{\LODilsixMass}{\SI{14}{pg/mL}}
\newcommand{\ECilten}{\SI{0.8}{pM}}
\newcommand{\ECilsix}{\SI{17}{pM}}

% ---- array statistics ----
\newcommand{\pxwell}{\num{2176}}
\newcommand{\rootN}{\num{47}}
\newcommand{\gmrep}{\SI{22}{\micro\siemens}}
\newcommand{\devcalib}{16\%}
\newcommand{\devraw}{62\%}

